Assaying Out-Of-Distribution Generalization in Transfer Learning

Since out-of-distribution generalization is a generally ill-posed problem, various proxy targets (e.g., calibration, adversarial robustness, algorithmic corruptions, invariance across shifts) were studied across different research programs resulting in different recommendations. While sharing the same aspirational goal, these approaches have never been tested under the same experimental conditions on real data. In this paper, we take a unified view of previous work, highlighting message discrepancies that we address empirically, and providing recommendations on how to measure the robustness of a model and how to improve it. To this end, we collect 172 publicly available dataset pairs for training and out-of-distribution evaluation of accuracy, calibration error, adversarial attacks, environment invariance, and synthetic corruptions. We fine-tune over 31k networks, from nine different architectures in the many- and few-shot setting. Our findings confirm that in- and out-of-distribution accuracies tend to increase jointly, but show that their relation is largely dataset-dependent, and in general more nuanced and more complex than posited by previous, smaller scale studies.

==> paper (status 10-21-2022)_arXiv/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm,bbm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\newcommand{\given}{\, \vert \,}
\def\vbeta{{\bm{\beta}}}
\def\vsigma{{\bm{\sigma}}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\indicator}{\mathbbm{1}}

==> paper (status 10-21-2022)_arXiv/tables/ID_OOD_gap_augmentation_selected_on_ID.tex <==
\begin{longtable}{llccc}
\caption{Average ID and OOD accuracy of each model on each task over all domains in the task.} \label{tab:model_comparison} \\
\toprule
        Model &           Domain &                            ID Error &                           OOD Error &                           OOD-ID Gap \\
\midrule
\endfirsthead

\toprule
        Model &           Domain &                            ID Error &                           OOD Error &                           OOD-ID Gap \\
\midrule
\endhead
\midrule
\multicolumn{5}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
\midrule
         Deit &             PACS & 0.033 \textcolor{gray}{$\pm$ 0.003} & 0.333 \textcolor{gray}{$\pm$ 0.022} &  0.299 \textcolor{gray}{$\pm$ 0.023} \\
              &             VLCS & 0.118 \textcolor{gray}{$\pm$ 0.010} & 0.328 \textcolor{gray}{$\pm$ 0.017} &  0.210 \textcolor{gray}{$\pm$ 0.022} \\
              &      domain\_net & 0.316 \textcolor{gray}{$\pm$ 0.009} & 0.703 \textcolor{gray}{$\pm$ 0.014} &  0.387 \textcolor{gray}{$\pm$ 0.017} \\
              &     office\_home & 0.131 \textcolor{gray}{$\pm$ 0.008} & 0.341 \textcolor{gray}{$\pm$ 0.017} &  0.209 \textcolor{gray}{$\pm$ 0.020} \\
              &            sviro & 0.014 \textcolor{gray}{$\pm$ 0.001} & 0.219 \textcolor{gray}{$\pm$ 0.005} &  0.205 \textcolor{gray}{$\pm$ 0.005} \\
              & terra\_incognita & 0.127 \textcolor{gray}{$\pm$ 0.011} & 0.661 \textcolor{gray}{$\pm$ 0.013} &  0.533 \textcolor{gray}{$\pm$ 0.020} \\
              & wilds-camelyon17 & 0.022 \textcolor{gray}{$\pm$ 0.007} & 0.156 \textcolor{gray}{$\pm$ 0.036} &  0.134 \textcolor{gray}{$\pm$ 0.040} \\
              &       wilds-fmow & 0.468 \textcolor{gray}{$\pm$ 0.036} & 0.543 \textcolor{gray}{$\pm$ 0.030} &  0.074 \textcolor{gray}{$\pm$ 0.007} \\
              &   wilds-iwildcam & 0.275 \textcolor{gray}{$\pm$ 0.007} & 0.289 \textcolor{gray}{$\pm$ 0.009} &  0.014 \textcolor{gray}{$\pm$ 0.006} \\
              &      wilds-rxrx1 & 0.925 \textcolor{gray}{$\pm$ 0.005} & 0.939 \textcolor{gray}{$\pm$ 0.004} &  0.014 \textcolor{gray}{$\pm$ 0.002} \\
\midrule
  DenseNet169 &             PACS & 0.061 \textcolor{gray}{$\pm$ 0.006} & 0.523 \textcolor{gray}{$\pm$ 0.031} &  0.463 \textcolor{gray}{$\pm$ 0.031} \\
              &             VLCS & 0.137 \textcolor{gray}{$\pm$ 0.011} & 0.365 \textcolor{gray}{$\pm$ 0.018} &  0.228 \textcolor{gray}{$\pm$ 0.024} \\
              &      domain\_net & 0.387 \textcolor{gray}{$\pm$ 0.011} & 0.788 \textcolor{gray}{$\pm$ 0.012} &  0.401 \textcolor{gray}{$\pm$ 0.015} \\
              &     office\_home & 0.209 \textcolor{gray}{$\pm$ 0.010} & 0.496 \textcolor{gray}{$\pm$ 0.017} &  0.287 \textcolor{gray}{$\pm$ 0.019} \\
              &            sviro & 0.047 \textcolor{gray}{$\pm$ 0.003} & 0.274 \textcolor{gray}{$\pm$ 0.005} &  0.227 \textcolor{gray}{$\pm$ 0.006} \\
              & terra\_incognita & 0.186 \textcolor{gray}{$\pm$ 0.015} & 0.725 \textcolor{gray}{$\pm$ 0.015} &  0.539 \textcolor{gray}{$\pm$ 0.019} \\
              & wilds-camelyon17 & 0.036 \textcolor{gray}{$\pm$ 0.012} & 0.169 \textcolor{gray}{$\pm$ 0.038} &  0.133 \textcolor{gray}{$\pm$ 0.047} \\
              &       wilds-fmow & 0.526 \textcolor{gray}{$\pm$ 0.046} & 0.593 \textcolor{gray}{$\pm$ 0.037} &  0.067 \textcolor{gray}{$\pm$ 0.009} \\
              &   wilds-iwildcam & 0.319 \textcolor{gray}{$\pm$ 0.010} & 0.364 \textcolor{gray}{$\pm$ 0.012} &  0.046 \textcolor{gray}{$\pm$ 0.021} \\
              &      wilds-rxrx1 & 0.911 \textcolor{gray}{$\pm$ 0.039} & 0.937 \textcolor{gray}{$\pm$ 0.027} &  0.026 \textcolor{gray}{$\pm$ 0.014} \\
\midrule
EfficientNet2 &             PACS & 0.053 \textcolor{gray}{$\pm$ 0.005} & 0.469 \textcolor{gray}{$\pm$ 0.032} &  0.416 \textcolor{gray}{$\pm$ 0.032} \\
              &             VLCS & 0.140 \textcolor{gray}{$\pm$ 0.012} & 0.374 \textcolor{gray}{$\pm$ 0.018} &  0.234 \textcolor{gray}{$\pm$ 0.023} \\
              &      domain\_net & 0.369 \textcolor{gray}{$\pm$ 0.012} & 0.734 \textcolor{gray}{$\pm$ 0.014} &  0.365 \textcolor{gray}{$\pm$ 0.017} \\
              &     office\_home & 0.172 \textcolor{gray}{$\pm$ 0.009} & 0.403 \textcolor{gray}{$\pm$ 0.015} &  0.230 \textcolor{gray}{$\pm$ 0.017} \\
              &            sviro & 0.031 \textcolor{gray}{$\pm$ 0.002} & 0.249 \textcolor{gray}{$\pm$ 0.005} &  0.218 \textcolor{gray}{$\pm$ 0.005} \\
              & terra\_incognita & 0.187 \textcolor{gray}{$\pm$ 0.016} & 0.703 \textcolor{gray}{$\pm$ 0.013} &  0.516 \textcolor{gray}{$\pm$ 0.017} \\
              & wilds-camelyon17 & 0.039 \textcolor{gray}{$\pm$ 0.015} & 0.194 \textcolor{gray}{$\pm$ 0.039} &  0.155 \textcolor{gray}{$\pm$ 0.049} \\
              &       wilds-fmow & 0.530 \textcolor{gray}{$\pm$ 0.053} & 0.588 \textcolor{gray}{$\pm$ 0.047} &  0.059 \textcolor{gray}{$\pm$ 0.006} \\
              &   wilds-iwildcam & 0.325 \textcolor{gray}{$\pm$ 0.022} & 0.383 \textcolor{gray}{$\pm$ 0.017} &  0.058 \textcolor{gray}{$\pm$ 0.009} \\
              &      wilds-rxrx1 & 0.901 \textcolor{gray}{$\pm$ 0.032} & 0.927 \textcolor{gray}{$\pm$ 0.022} &  0.025 \textcolor{gray}{$\pm$ 0.013} \\
\midrule
         GMLP &             PACS & 0.070 \textcolor{gray}{$\pm$ 0.007} & 0.434 \textcolor{gray}{$\pm$ 0.026} &  0.363 \textcolor{gray}{$\pm$ 0.027} \\
              &             VLCS & 0.136 \textcolor{gray}{$\pm$ 0.011} & 0.361 \textcolor{gray}{$\pm$ 0.016} &  0.225 \textcolor{gray}{$\pm$ 0.022} \\
              &      domain\_net & 0.404 \textcolor{gray}{$\pm$ 0.012} & 0.753 \textcolor{gray}{$\pm$ 0.013} &  0.348 \textcolor{gray}{$\pm$ 0.017} \\
              &     office\_home & 0.195 \textcolor{gray}{$\pm$ 0.009} & 0.409 \textcolor{gray}{$\pm$ 0.016} &  0.214 \textcolor{gray}{$\pm$ 0.020} \\
              &            sviro & 0.034 \textcolor{gray}{$\pm$ 0.002} & 0.260 \textcolor{gray}{$\pm$ 0.006} &  0.226 \textcolor{gray}{$\pm$ 0.006} \\
              & terra\_incognita & 0.180 \textcolor{gray}{$\pm$ 0.016} & 0.708 \textcolor{gray}{$\pm$ 0.010} &  0.528 \textcolor{gray}{$\pm$ 0.021} \\
              & wilds-camelyon17 & 0.041 \textcolor{gray}{$\pm$ 0.016} & 0.214 \textcolor{gray}{$\pm$ 0.032} &  0.173 \textcolor{gray}{$\pm$ 0.042} \\
              &       wilds-fmow & 0.556 \textcolor{gray}{$\pm$ 0.056} & 0.624 \textcolor{gray}{$\pm$ 0.046} &  0.069 \textcolor{gray}{$\pm$ 0.011} \\
              &   wilds-iwildcam & 0.338 \textcolor{gray}{$\pm$ 0.009} & 0.329 \textcolor{gray}{$\pm$ 0.006} & -0.008 \textcolor{gray}{$\pm$ 0.011} \\
              &      wilds-rxrx1 & 0.972 \textcolor{gray}{$\pm$ 0.008} & 0.977 \textcolor{gray}{$\pm$ 0.006} &  0.005 \textcolor{gray}{$\pm$ 0.002} \\
\midrule
        Mixer &             PACS & 0.091 \textcolor{gray}{$\pm$ 0.009} & 0.469 \textcolor{gray}{$\pm$ 0.028} &  0.378 \textcolor{gray}{$\pm$ 0.029} \\
              &             VLCS & 0.150 \textcolor{gray}{$\pm$ 0.011} & 0.386 \textcolor{gray}{$\pm$ 0.017} &  0.236 \textcolor{gray}{$\pm$ 0.022} \\
              &      domain\_net & 0.433 \textcolor{gray}{$\pm$ 0.014} & 0.785 \textcolor{gray}{$\pm$ 0.012} &  0.352 \textcolor{gray}{$\pm$ 0.016} \\
              &     office\_home & 0.215 \textcolor{gray}{$\pm$ 0.011} & 0.472 \textcolor{gray}{$\pm$ 0.016} &  0.257 \textcolor{gray}{$\pm$ 0.020} \\
              &            sviro & 0.023 \textcolor{gray}{$\pm$ 0.001} & 0.251 \textcolor{gray}{$\pm$ 0.005} &  0.228 \textcolor{gray}{$\pm$ 0.005} \\
              & terra\_incognita & 0.172 \textcolor{gray}{$\pm$ 0.015} & 0.737 \textcolor{gray}{$\pm$ 0.013} &  0.565 \textcolor{gray}{$\pm$ 0.018} \\
              & wilds-camelyon17 & 0.025 \textcolor{gray}{$\pm$ 0.008} & 0.154 \textcolor{gray}{$\pm$ 0.029} &  0.129 \textcolor{gray}{$\pm$ 0.036} \\
              &       wilds-fmow & 0.534 \textcolor{gray}{$\pm$ 0.042} & 0.608 \textcolor{gray}{$\pm$ 0.038} &  0.074 \textcolor{gray}{$\pm$ 0.005} \\
              &   wilds-iwildcam & 0.333 \textcolor{gray}{$\pm$ 0.005} & 0.374 \textcolor{gray}{$\pm$ 0.009} &  0.041 \textcolor{gray}{$\pm$ 0.012} \\
              &      wilds-rxrx1 & 0.983 \textcolor{gray}{$\pm$ 0.006} & 0.985 \textcolor{gray}{$\pm$ 0.005} &  0.002 \textcolor{gray}{$\pm$ 0.001} \\
\midrule
       ResMLP &             PACS & 0.066 \textcolor{gray}{$\pm$ 0.006} & 0.465 \textcolor{gray}{$\pm$ 0.026} &  0.398 \textcolor{gray}{$\pm$ 0.026} \\
              &             VLCS & 0.145 \textcolor{gray}{$\pm$ 0.011} & 0.395 \textcolor{gray}{$\pm$ 0.017} &  0.250 \textcolor{gray}{$\pm$ 0.022} \\
              &      domain\_net & 0.398 \textcolor{gray}{$\pm$ 0.011} & 0.764 \textcolor{gray}{$\pm$ 0.012} &  0.367 \textcolor{gray}{$\pm$ 0.016} \\
              &     office\_home & 0.203 \textcolor{gray}{$\pm$ 0.010} & 0.453 \textcolor{gray}{$\pm$ 0.018} &  0.250 \textcolor{gray}{$\pm$ 0.021} \\
              &            sviro & 0.027 \textcolor{gray}{$\pm$ 0.001} & 0.245 \textcolor{gray}{$\pm$ 0.005} &  0.218 \textcolor{gray}{$\pm$ 0.005} \\
              & terra\_incognita & 0.164 \textcolor{gray}{$\pm$ 0.014} & 0.694 \textcolor{gray}{$\pm$ 0.013} &  0.530 \textcolor{gray}{$\pm$ 0.020} \\
              & wilds-camelyon17 & 0.032 \textcolor{gray}{$\pm$ 0.012} & 0.157 \textcolor{gray}{$\pm$ 0.015} &  0.125 \textcolor{gray}{$\pm$ 0.025} \\
              &       wilds-fmow & 0.544 \textcolor{gray}{$\pm$ 0.047} & 0.613 \textcolor{gray}{$\pm$ 0.039} &  0.069 \textcolor{gray}{$\pm$ 0.009} \\
              &   wilds-iwildcam & 0.317 \textcolor{gray}{$\pm$ 0.006} & 0.343 \textcolor{gray}{$\pm$ 0.009} &  0.026 \textcolor{gray}{$\pm$ 0.008} \\
              &      wilds-rxrx1 & 0.949 \textcolor{gray}{$\pm$ 0.010} & 0.959 \textcolor{gray}{$\pm$ 0.005} &  0.010 \textcolor{gray}{$\pm$ 0.005} \\
\midrule
     ResNet50 &             PACS & 0.054 \textcolor{gray}{$\pm$ 0.005} & 0.499 \textcolor{gray}{$\pm$ 0.032} &  0.445 \textcolor{gray}{$\pm$ 0.033} \\
              &             VLCS & 0.137 \textcolor{gray}{$\pm$ 0.011} & 0.325 \textcolor{gray}{$\pm$ 0.017} &  0.189 \textcolor{gray}{$\pm$ 0.022} \\
              &      domain\_net & 0.359 \textcolor{gray}{$\pm$ 0.011} & 0.749 \textcolor{gray}{$\pm$ 0.014} &  0.390 \textcolor{gray}{$\pm$ 0.016} \\
              &     office\_home & 0.180 \textcolor{gray}{$\pm$ 0.010} & 0.431 \textcolor{gray}{$\pm$ 0.017} &  0.251 \textcolor{gray}{$\pm$ 0.020} \\
              &            sviro & 0.025 \textcolor{gray}{$\pm$ 0.001} & 0.244 \textcolor{gray}{$\pm$ 0.005} &  0.220 \textcolor{gray}{$\pm$ 0.006} \\
              & terra\_incognita & 0.176 \textcolor{gray}{$\pm$ 0.014} & 0.698 \textcolor{gray}{$\pm$ 0.015} &  0.521 \textcolor{gray}{$\pm$ 0.019} \\
              & wilds-camelyon17 & 0.036 \textcolor{gray}{$\pm$ 0.013} & 0.195 \textcolor{gray}{$\pm$ 0.045} &  0.159 \textcolor{gray}{$\pm$ 0.052} \\
              &       wilds-fmow & 0.512 \textcolor{gray}{$\pm$ 0.045} & 0.579 \textcolor{gray}{$\pm$ 0.036} &  0.067 \textcolor{gray}{$\pm$ 0.010} \\
              &   wilds-iwildcam & 0.313 \textcolor{gray}{$\pm$ 0.015} & 0.328 \textcolor{gray}{$\pm$ 0.007} &  0.015 \textcolor{gray}{$\pm$ 0.010} \\
              &      wilds-rxrx1 & 0.894 \textcolor{gray}{$\pm$ 0.032} & 0.925 \textcolor{gray}{$\pm$ 0.021} &  0.030 \textcolor{gray}{$\pm$ 0.012} \\
\midrule
         Swin &             PACS & 0.048 \textcolor{gray}{$\pm$ 0.006} & 0.393 \textcolor{gray}{$\pm$ 0.027} &  0.345 \textcolor{gray}{$\pm$ 0.027} \\
              &             VLCS & 0.121 \textcolor{gray}{$\pm$ 0.010} & 0.350 \textcolor{gray}{$\pm$ 0.017} &  0.230 \textcolor{gray}{$\pm$ 0.021} \\
              &      domain\_net & 0.340 \textcolor{gray}{$\pm$ 0.010} & 0.718 \textcolor{gray}{$\pm$ 0.014} &  0.378 \textcolor{gray}{$\pm$ 0.017} \\
              &     office\_home & 0.152 \textcolor{gray}{$\pm$ 0.009} & 0.351 \textcolor{gray}{$\pm$ 0.018} &  0.199 \textcolor{gray}{$\pm$ 0.022} \\
              &            sviro & 0.019 \textcolor{gray}{$\pm$ 0.001} & 0.218 \textcolor{gray}{$\pm$ 0.005} &  0.199 \textcolor{gray}{$\pm$ 0.005} \\
              & terra\_incognita & 0.144 \textcolor{gray}{$\pm$ 0.012} & 0.643 \textcolor{gray}{$\pm$ 0.013} &  0.498 \textcolor{gray}{$\pm$ 0.019} \\
              & wilds-camelyon17 & 0.026 \textcolor{gray}{$\pm$ 0.010} & 0.137 \textcolor{gray}{$\pm$ 0.020} &  0.111 \textcolor{gray}{$\pm$ 0.028} \\
              &       wilds-fmow & 0.481 \textcolor{gray}{$\pm$ 0.053} & 0.548 \textcolor{gray}{$\pm$ 0.045} &  0.067 \textcolor{gray}{$\pm$ 0.008} \\
              &   wilds-iwildcam & 0.290 \textcolor{gray}{$\pm$ 0.004} & 0.282 \textcolor{gray}{$\pm$ 0.004} & -0.007 \textcolor{gray}{$\pm$ 0.004} \\
              &      wilds-rxrx1 & 0.875 \textcolor{gray}{$\pm$ 0.042} & 0.905 \textcolor{gray}{$\pm$ 0.027} &  0.029 \textcolor{gray}{$\pm$ 0.016} \\
\midrule
        ViT-B &             PACS & 0.063 \textcolor{gray}{$\pm$ 0.008} & 0.415 \textcolor{gray}{$\pm$ 0.027} &  0.352 \textcolor{gray}{$\pm$ 0.027} \\
              &             VLCS & 0.137 \textcolor{gray}{$\pm$ 0.011} & 0.341 \textcolor{gray}{$\pm$ 0.017} &  0.205 \textcolor{gray}{$\pm$ 0.020} \\
              &      domain\_net & 0.378 \textcolor{gray}{$\pm$ 0.013} & 0.736 \textcolor{gray}{$\pm$ 0.014} &  0.357 \textcolor{gray}{$\pm$ 0.017} \\
              &     office\_home & 0.163 \textcolor{gray}{$\pm$ 0.011} & 0.367 \textcolor{gray}{$\pm$ 0.019} &  0.204 \textcolor{gray}{$\pm$ 0.023} \\
              &            sviro & 0.023 \textcolor{gray}{$\pm$ 0.001} & 0.223 \textcolor{gray}{$\pm$ 0.006} &  0.200 \textcolor{gray}{$\pm$ 0.006} \\
              & terra\_incognita & 0.155 \textcolor{gray}{$\pm$ 0.012} & 0.697 \textcolor{gray}{$\pm$ 0.011} &  0.542 \textcolor{gray}{$\pm$ 0.018} \\
              & wilds-camelyon17 & 0.024 \textcolor{gray}{$\pm$ 0.007} & 0.148 \textcolor{gray}{$\pm$ 0.022} &  0.124 \textcolor{gray}{$\pm$ 0.029} \\
              &       wilds-fmow & 0.495 \textcolor{gray}{$\pm$ 0.038} & 0.565 \textcolor{gray}{$\pm$ 0.033} &  0.070 \textcolor{gray}{$\pm$ 0.006} \\
              &   wilds-iwildcam & 0.303 \textcolor{gray}{$\pm$ 0.006} & 0.334 \textcolor{gray}{$\pm$ 0.021} &  0.031 \textcolor{gray}{$\pm$ 0.017} \\
              &      wilds-rxrx1 & 0.951 \textcolor{gray}{$\pm$ 0.013} & 0.966 \textcolor{gray}{$\pm$ 0.008} &  0.015 \textcolor{gray}{$\pm$ 0.005} \\
\end{longtable}


==> paper (status 10-21-2022)_arXiv/tables/ID_OOD_gap_small_error.tex <==
\begin{longtable}{lccc}
\toprule
        Model &                            ID Error &                           OOD Error &                          OOD-ID Gap \\
\midrule
\endfirsthead

\toprule
        Model &                            ID Error &                           OOD Error &                          OOD-ID Gap \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
         Deit & \textbf{0.101} \textcolor{gray}{$\pm$ 0.005} & \textbf{0.364} \textcolor{gray}{$\pm$ 0.008} & 0.263 \textcolor{gray}{$\pm$ 0.006} \\
         Swin & 0.111 \textcolor{gray}{$\pm$ 0.005} & 0.371 \textcolor{gray}{$\pm$ 0.008} & \textbf{0.260} \textcolor{gray}{$\pm$ 0.006} \\
        ViT-B & 0.124 \textcolor{gray}{$\pm$ 0.005} & 0.384 \textcolor{gray}{$\pm$ 0.008} & 0.259 \textcolor{gray}{$\pm$ 0.006} \\
     ResNet50 & 0.124 \textcolor{gray}{$\pm$ 0.005} & 0.406 \textcolor{gray}{$\pm$ 0.008} & 0.283 \textcolor{gray}{$\pm$ 0.006} \\
EfficientNet2 & 0.129 \textcolor{gray}{$\pm$ 0.005} & 0.407 \textcolor{gray}{$\pm$ 0.008} & 0.277 \textcolor{gray}{$\pm$ 0.006} \\
         GMLP & 0.140 \textcolor{gray}{$\pm$ 0.006} & 0.413 \textcolor{gray}{$\pm$ 0.008} & 0.273 \textcolor{gray}{$\pm$ 0.006} \\
       ResMLP & 0.134 \textcolor{gray}{$\pm$ 0.005} & 0.413 \textcolor{gray}{$\pm$ 0.008} & 0.279 \textcolor{gray}{$\pm$ 0.006} \\
        Mixer & 0.142 \textcolor{gray}{$\pm$ 0.006} & 0.425 \textcolor{gray}{$\pm$ 0.008} & 0.282 \textcolor{gray}{$\pm$ 0.006} \\
  DenseNet169 & 0.145 \textcolor{gray}{$\pm$ 0.005} & 0.443 \textcolor{gray}{$\pm$ 0.008} & 0.298 \textcolor{gray}{$\pm$ 0.006} \\
\end{longtable}

